Embodied Evolution in Collective Robotics: A Review

This paper provides an overview of evolutionary robotics techniques applied to on-line distributed evolution for robot collectives -- namely, embodied evolution. It provides a definition of embodied evolution as well as a thorough description of the underlying concepts and mechanisms. The paper also presents a comprehensive summary of research published in the field since its inception (1999-2017), providing various perspectives to identify the major trends. In particular, we identify a shift from considering embodied evolution as a parallel search method within small robot collectives (fewer than 10 robots) to embodied evolution as an on-line distributed learning method for designing collective behaviours in swarm-like collectives. The paper concludes with a discussion of applications and open questions, providing a milestone for past and an inspiration for future research.

==> glossary.tex <==
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% DO NOT UPDATE THIS FILE FROM 2017/11/30 %%%% %%%% %%%% %%%% 
%%%% %%%% ORIGINAL GLOSSARY IS IN MAIN.TEX   %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% AS THIS IS MANDATORY FOR FRONTIERS SUBMISSION %%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 


% !TEX root = main.tex
\setlength{\extrarowheight}{0.1cm}
\begin{table}[ht]
\centering
\begin{tabular}{lp{10cm}}%>{\itshape}p{7cm}}
\toprule
\textbf{Field} & %\textbf{Value} & 
\textbf{Comment} \\
\midrule
Implementation & \textbf{Distributed} implementations have one genome for each robot, and an offspring is created only as the result of a mating event or by mutating the current genome. \textbf{Hybrid} implementations have multiple genomes per robot, and offspring can be created from this internal pool as well as from genomes `imported' through mating events. As stated earlier, the encapsulated scheme is not considered embodied evolution as there is no exchange of genomes between robots in this case.\\
%\hline
 & The experiments can use \textbf{real robots} or \textbf{simulation}.\\
%\hline
Robot behaviour & 
A \textbf{monomorphic} population contains individuals with similar genotypes (with variations due to mutation). A \textbf{polymorphic} population is divided into two (or more) subgroups of genetically similar individuals, and different genotypic signatures from one group to the other, e.g., to achieve specialisation.\\
%\hline
 & We distinguish between experiments that target efficient \textbf{individual behaviour} vs. collective behaviours (i.e., social behaviours, incl. cooperation) \\
%\hline
Experimental settings & Identifies the \textbf{task(s)} considered in the experiment, e.g., obstacle avoidance, foraging, ... \textbf{None} indicates that there is no user-defined task and that consequently, selection pressure results from the environment only. 
The \textbf{number of robots} used is also included. $n_1-n_2$ indicates the interval for one experiment and $n1;n2$ gives numbers for two experiments.\\
%\hline
Mating conditions & Mating can be based on \textbf{proximity}: two robots can mate whenever they are physically close to each other (e.g., in infrared communication range). In \textbf{panmictic} systems, robots can mate with all other robots, regardless of their location. \textbf{Other} comprises of systems where robots maintain an explicit list of potential mates (a social network) which may be maintained through gossiping.  \\
%\hline
Selection scheme & Parents are selected from the received and internal genomes on the basis of their \textbf{performance} if a task is defined. \textbf{Random} parent selection implies only environment-driven selection. Currently, the only examples of \textbf{other} selection schemes use genotypic distance, but this category also covers metrics such as novelty. \\
%\hline
Replacement scheme & Genomes can have a \textbf{fixed lifetime}, \textbf{variable lifetime} or \textbf{limited lifetime} (similar to variable lifetime, but with an upper bound). \textbf{Event\hyp{}based} replacement schemes do not depend on time, but on events such as reception of genetic material (e.g. in the microbial GA used by \citet{Watson2002a}).  \\
\bottomrule
\end{tabular}
\caption{Glossary}
\label{tab:glossary}
\end{table}


==> table.tex <==
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% DO NOT UPDATE THIS FILE FROM 2017/11/30 %%%% %%%% %%%% %%%% 
%%%% %%%% ORIGINAL TABLE IS IN MAIN.TEX %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% AS THIS IS MANDATORY FOR FRONTIERS SUBMISSION %%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 
%%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% %%%% 




% !TEX root = main.tex

\newcolumntype{R}[2]{%
    >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
    c%
    <{\egroup}%
}
\newcommand*\rot{\multicolumn{1}{R{-90}{.01cm}}}
\newcommand*\Yes{$\bullet$}

\begin{sidewaystable}[t]
\scriptsize
\begin{center}
\begin{tabular}{p{2in}p{.01cm}p{.01cm}p{.01cm}p{.01cm}cccccp{1.2in}lcccccccccc}
\toprule
%&\multicolumn{2}{l}{}%Scheme}
\multicolumn{5}{r}{Implementation}
&\multicolumn{5}{|c}{Robot Behaviour}
&\multicolumn{2}{|c}{Experimental Settings}
%&%nr of robots
&\multicolumn{3}{|c}{Mating Conditions}
&\multicolumn{3}{|c}{Selection Scheme}
&\multicolumn{4}{|c}{Replacement Scheme}
%&\multicolumn{2}{c}{Phenotype}
\\ \midrule

&\rot{distributed}&\rot{hybrid}
&\rot{simulation}&\rot{real robots}
&\rot{monomorphic}&\rot{polymorphic}
&\rot{individual behaviour}&\rot{cooperation}&\rot{division of labour}
&\rot{task}~%\rot{foraging}&\rot{agreggation}&\rot{surveillance}&\rot{prey}&\rot{predator}&\rot{phototaxis}&\rot{items avoidance}&\rot{navigation}&\rot{synthetic mapping}
&\rot{nr of robots}
&\rot{panmictic}&\rot{proximity}&\rot{other}
%&\rot{\cellcolor{black!15}gossiping}
&\rot{performance}&\rot{random}&\rot{genotypic distance}
&\rot{fixed lifetime}&\rot{variable lifetime}&\rot{event-based}&\rot{limited lifetime}
%if we add phenotype columns: E.g. Controller (NN) or Morphology (sensor layout)
\\
%\midrule

\rowcolor{black!15}
\cite{Ficici1999,Watson2002a} %		distributed	real robots	monomorphic, individual behaviour	phototaxis	static	8	homogeneous	partially connected (proximity)	performance	variable lifetime
&\Yes 	% distributed
&~ 		% hybrid
&~		% simulation
&\Yes	% real robots
&\Yes	% monomorphic
&~		% polymorphic
&\Yes	% individual behaviour
&~		% cooperation
&~		% division of labour
&phototaxis % Task
&8 		%nr robots
% mating:
&~		% panmictic
&\Yes	% distance-based
&~		% social network
		% gossiping
%parent selection: 
&\Yes	% performance-based
&~		% random
&~		% genotypic proximity
% replacement: 
&		% fixed lifetime
&\Yes	% variable lifetime
&~		% event-based
&~		% upper-bounded lifetime
\\

\cite{Simoes2001}	%	distributed	real robots	monomorphic, individual behaviour	obstacle avoidance	static	6	variable	fully connected	performance	limited lifetime
&\Yes&~ %distributed, hybrid
&~&\Yes %simulation, real robots
&\Yes&~&\Yes&&~% monomorphic; polymorphic; individual behaviour; cooperation; division of labour
&obstacle avoidance
&6 %nr robots
&\Yes&~&~ % mating: panmictic; distance-based; social network; gossiping
&\Yes&~&~ % parent selection: performance-based; random; genotypic proximity
&\Yes&~&~&~ % replacement: fixed lifetime; variable lifetime; event-based; upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Usui2003Situated-and-Em}	%	hybrid	real robots	monomorphic, individual behaviour	obstacle avoidance	static	6	homogeneous	partially connected (proximity)	performance	fixed lifetime
&	 	% distributed
&\Yes	% hybrid
&~		% simulation
&\Yes	% real robots
&\Yes	% monomorphic
&~		% polymorphic
&\Yes	% individual behaviour
&~		% cooperation
&~		% division of labour
&obstacle avoidance % Task
&6 		%nr robots
% mating:
&~		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&~		% random
&~		% genotypic proximity
% replacement: 
&\Yes	% fixed lifetime
&		% variable lifetime
&~		% event-based
&~		% upper-bounded lifetime
\\

\cite{Bianco2004}%		distributed	simulation	monomorphic, individual behaviour	self-assembling	static	64	homogeneous	partially connected (contact-based)	relative location wrt. partner	event-based
&\Yes 	% distributed
&		% hybrid
&\Yes	% simulation
&		% real robots
&\Yes	% monomorphic
&~		% polymorphic
&\Yes	% individual behaviour
&~		% cooperation
&~		% division of labour
&self assembly % Task
&64		%nr robots
% mating:
&~		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&~		% performance-based
&\Yes	% random
&		% genotypic proximity
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&\Yes	% event-based
&~		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Hettiarachchi2006,Hettiarachchi2009a}	% distributed	simulation	individual behaviour	navigation with obstacle avoidance	60	homogeneous	static	partially connected (proximity)	performance
&\Yes		% distributed
&		% hybrid
&\Yes	% simulation
&		% real robots
&\Yes 	% monomorphic
&~		% polymorphic
&\Yes	% individual behaviour
&~		% cooperation
&~		% division of labour
&navigation with obstacle avoidance % Task
&60	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&~		% random
&~		% genotypic proximity\todo{selection is "relative location wrt. partner"... add `other' category?}
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&\Yes		% event-based
&~		% upper-bounded lifetime
\\

\cite{Wischmann2007Embodied-evolut}	%	distributed	simulation	monomorphic, individual behaviour	foraging as a proxy for predator avoidance	static	3 (+3 non-evolving)	homogeneous	partially connected (proximity)	performance	variable time
&\Yes&~ %distributed, hybrid
&\Yes&~ %simulation, real robots
&\Yes&~&\Yes&~&~% monomorphic; polymorphic; individual behaviour; cooperation; division of labour
&foraging$^1$
&3%nr robots
&~&\Yes&~%&~ % mating: panmictic; distance-based; social network; gossiping
&\Yes&~&~ % parent selection: performance-based; random; genotypic proximity
&~&\Yes&~&~ % replacement: fixed lifetime; variable lifetime; event-based; upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Perez2008Embodied-Evolut}	%hybrid	simulation	individual behaviour	obstacle avoidance	5	homogeneous	static	fully connected	performance
& 		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&		% real robots
&\Yes 	% monomorphic
&~		% polymorphic
&\Yes	% individual behaviour
&~		% cooperation
&~		% division of labour
&obstacle avoidance % Task
&5		%nr robots
% mating:
&\Yes	% panmictic
&		% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&~		% random
&~		% genotypic proximity\todo{selection is "relative location wrt. partner"... add `other' category?}
% replacement: 
&\Yes	% fixed lifetime (fixed generation-like time)
&		% variable lifetime
&		% event-based
&~		% upper-bounded lifetime
\\

\cite{Konig2009a,Konig2009b}%distributed	simulation	individual behaviour	obstacle avoidance & gate passing	26;30	homogeneous	static	partially connected (proximity)	performance
&\Yes		% distributed
&		% hybrid
&\Yes	% simulation
&		% real robots
&\Yes 	% monomorphic
&~		% polymorphic
&\Yes	% individual behaviour
&~		% cooperation
&~		% division of labour
&obstacle avoidance with gate passing % Task
&26;30	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&~		% random
&~		% genotypic proximity\todo{selection is "relative location wrt. partner"... add `other' category?}
% replacement: 
&\Yes	% fixed lifetime (cf. p18 of paper)
&		% variable lifetime
&		% event-based
&~		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Pugh2009} %	hybrid	simulation & real robots	individual behaviour	obstacle avoidance	1, 2, 5, and 10	homogeneous	static	comparison between fully connected and partially connected (proximity)	performance
&		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&\Yes	% real robots
&\Yes 	% monomorphic
&~		% polymorphic
&\Yes	% individual behaviour
&~		% cooperation
&~		% division of labour
&obstacle avoidance% Task
&1--10	%nr robots
% mating:
&\Yes		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&~		% random
&~		% genotypic proximity\todo{selection is "relative location wrt. partner"... add `other' category?}
% replacement: 
&\Yes	% fixed lifetime
&		% variable lifetime
&		% event-based
&~		% upper-bounded lifetime
\\

\cite{Prieto2009,Trueba2011,Trueba2012a}	%distributed	Simulated	polimorphic, collective behaviour	surveillance / foraging / construction	static	20	homogeneous	Partially connected (proximity)	performance	limited lifetime; event-based
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
& 	% monomorphic
&\Yes		% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&\Yes		% division of labour
&surveillance, foraging, construction% Task
&20	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&~		% random
&~		% genotypic proximity\todo{selection is "relative location wrt. partner"... add `other' category?}
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&\Yes		% event-based
&\Yes		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{bredeche2010ppsn,Bredeche2012,bredeche2014alife}	%	distributed	real robots ; simulation	monomorphic, cooperation	none	dynamic	20; 4000	homogeneous	partially connected (proximity)	random	upper-bounded lifetime
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&\Yes	% real robots
&\Yes 	% monomorphic
&		% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&~		% division of labour
&none% Task
&20;4000	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&	% performance-based
&\Yes		% random
&~		% genotypic proximity\todo{selection is "relative location wrt. partner"... add `other' category?}
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&		% event-based
&\Yes		% upper-bounded lifetime
\\

\cite{Prieto2010}	%distributed	Real robots	polimorphic, collective behaviour	surveillance	static; dynamic	8	homogeneous	Partially connected (proximity)	performance	limited lifetime; event-based
&\Yes		% distributed
&	% hybrid
&	% simulation
&\Yes	% real robots
& 	% monomorphic
&\Yes	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&\Yes		% division of labour
&surveillance% Task
&8	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&~		% genotypic proximity\todo{selection is "relative location wrt. partner"... add `other' category?}
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&\Yes		% event-based
&\Yes		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Schwarzer2010Artificial-Sexu} %	distributed	simulation & real robots	polymorphic collaboration	none	upto 40	homogeneous	static	partially-connected (proximity)	parental investment
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&\Yes	% real robots
& 	% monomorphic
&\Yes	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&~		% division of labour
&none% Task
&upto 40	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&	% performance-based
&\Yes		% random
&		% genotypic proximity\todo{selection is "parental investment"... add `other' category?}
% replacement: 
&		% fixed lifetime
&\Yes		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\cite{Schwarzer2011}%	distributed	simulation	monomorphic; individual behaviour	phototaxis	4	homogeneous	dynamic	partially connected (proximity)	performance
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&\Yes	% individual behaviour
&		% cooperation
&~		% division of labour
&phototaxis% Task
&4	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes	% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Montanier2011,montanier2013}%		distributed	simulation	monomorphic, cooperation	none	dynamic	100	homogeneous	partially connected (proximity)	random; genotypic proximity	upper-bounded lifetime
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&~		% division of labour
&none% Task
&100	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&	% performance-based
&\Yes		% random
&\Yes		% genotypic proximity
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&		% event-based
&\Yes		% upper-bounded lifetime
\\

\cite{Huijsman2011An-On-line-On-b} %	hybrid & distributed	simulation	monomorphic; individual behaviour	obstacle avoidance	4, 16, 36 and 400	homogeneous	static	fully connected or partially connected (gossiping)	performance
&\Yes		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&\Yes	% individual behaviour
&		% cooperation
&~		% division of labour
&obstacle avoidance% Task
&4--400	%nr robots
% mating:
&\Yes		% panmictic
&	% distance-based
%&~		% social network
&\Yes		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Karafotias2011An-Algorithm-fo}%	hybrid	simulation	monomorphic; individual behaviour	obstacle avoidance, phototaxis and patrolling	10	homogeneous	static	partially connected (social network)	performance
&		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&\Yes	% individual behaviour
&		% cooperation
&\Yes	% division of labour
&obstacle avoidance, phototaxis and patrolling% Task
&10	%nr robots
% mating:
&		% panmictic
&	% distance-based
&\Yes		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\cite{Silva2012,Silva2013a,Silva2015,Silva2017}	%distributed	Simulated	polimorphic, individual and collective behaviour	aggregation / surveillance	static	5 / 10 / 15 / 20	homogeneous	Partially connected (performance; proximity)	performance	event-based
&		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&\Yes	% real robots
& 	% monomorphic
&\Yes	% polymorphic
&\Yes	% individual behaviour
&\Yes		% cooperation
&~		% division of labour
&navigation, aggregation, surveillance, phototaxis% Task
&2--20	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&\Yes		% event-based
&		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{weel2012organisms,weel2012online}%	hybrid	simulation	monomorphic; cooperation	foraging	10 (first paper), 50 (2nd paper)	homogeneous	dynamic	partially connected (proximity)	performance
&		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&~		% division of labour
&foraging% Task
&10;50	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\cite{Garcia-Sanchez2012Testing-Diversi}%	hybrid	simulation	monomorphic; individual behaviour	obstacle avoidance	4, 16 and 36 robots	homogeneous	static	partially connected (social network or proximity)	performance
&		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&\Yes	% individual behaviour
&		% cooperation
&~		% division of labour
&obstacle avoidance% Task
&4--36	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&\Yes	% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Noskov2013a,Haasdijk2013,Haasdijk2013b,Haasdijk2014,Haasdijk2016,Kemeling2017,Bangel2017}%	distributed	simulation	polymorphic; division of labour	foraging	150	homogeneous	static	partially connected (proximity)	performance
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots\textbf{}
& 	% monomorphic
&\Yes	% polymorphic
&\Yes	% individual behaviour
&		% cooperation
&\Yes	% division of labour
&foraging% Task
&100	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\cite{Trueba2013682,Trueba2017}%	distributed	abstract; simulated; real robots	polimorphic, collective behaviour	synthetic mapping / gathering	static	20 / 9	homogeneous	fully connected	performance; random ; spatial proximity	limited lifetime; event-based
&\Yes	% distributed
&	% hybrid
&\Yes	% simulation
&\Yes	% real robots
& 	% monomorphic
&\Yes	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&\Yes~		% division of labour
&synthetic mapping, gathering, self-location% Task
&40;20;9	%nr robots
% mating:
&\Yes		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&\Yes		% random
&		% genotypic proximity
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&\Yes		% event-based
&\Yes		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{ODowd2014a}%	hybrid	real robots	monomorphic; individual behaviour	foraging	10	homogeneous	dynamic	partially connected (proximity)	performance of controller (co-evolution w controllers)
&		% distributed
&\Yes	% hybrid
&	% simulation
&\Yes	% real robots
& \Yes	% monomorphic
&	% polymorphic
&\Yes	% individual behaviour
&		% cooperation
&~		% division of labour
&foraging% Task
&10	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\cite{FernandezPerez2014}%		distributed	simulation	monomorphic, cooperation	foraging	static	50	homogeneous	partially connected (proximity)	performance; random	limited lifetime
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes	% monomorphic
&	% polymorphic
&	% individual behaviour
&		% cooperation
&\Yes		% division of labour
&foraging	% Task
&50	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&\Yes		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{FernandezPerez2015}%		distributed	simulation	monomorphic, cooperation	foraging	static	100	homogeneous	partially connected (proximity)	performance	event-based
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&~		% division of labour
&foraging% Task
&100	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&\Yes	% event-based
&		% upper-bounded lifetime
\\

\cite{Hart2015,Steyven2016}%		distributed	simulation	monomorphic, cooperation	foraging	static	100	homogeneous	partially connected (proximity)	performance	upper-bounded lifetime									
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&~		% division of labour
&foraging% Task
&100	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&		% event-based
&\Yes	% upper-bounded lifetime
\\

\rowcolor{black!15}
\cite{Heinerman2015-3foldadaptivity,Heinerman2015-3foldthymio}%	hybrid	simulation	monomorphic; individual behaviour	obstacle avoidance	6 robots	variable	static	panmictic	performance
&		% distributed
&\Yes	% hybrid
&\Yes	% simulation
&\Yes	% real robots
&\Yes 	% monomorphic
&	% polymorphic
&\Yes	% individual behaviour
&		% cooperation
&~		% division of labour
&obstacle avoidance% Task
&6	%nr robots
% mating:
&\Yes		% panmictic
&	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&		% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\

\cite{Montanier2016,Bredeche2017}%		distributed	simulation	polymorphic, division of labour	none	static	100-500	homogeneous	partially connected (proximity)	random; genotypic proximity	upper-bounded lifetime
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
&	% monomorphic
&\Yes 	% polymorphic
&	% individual behaviour
&		% cooperation
&\Yes		% division of labour
&foraging% Task
&100;500	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&\Yes	% random
&		% genotypic proximity
% replacement: 
&		% fixed lifetime
&		% variable lifetime
&		% event-based
&\Yes		% upper-bounded lifetime
\\
\rowcolor{black!15}
\cite{Perez2017}
&\Yes		% distributed
&	% hybrid
&\Yes	% simulation
&	% real robots
&	% monomorphic
&\Yes 	% polymorphic
&	% individual behaviour
&\Yes		% cooperation
&		% division of labour
&foraging% Task
&200	%nr robots
% mating:
&		% panmictic
&\Yes	% distance-based
&~		% social network
%&~		% gossiping
%parent selection: 
&\Yes	% performance-based
&	% random
&		% genotypic proximity
% replacement: 
&\Yes		% fixed lifetime
&		% variable lifetime
&		% event-based
&		% upper-bounded lifetime
\\
\bottomrule
%'footnotes' for table at the bottom.
\multicolumn{8}{l}{%\footnotesize
$^1$ as a proxy for predator avoidance}\\
\end{tabular}
\end{center}
\caption{Overview of Embodied Evolution research}
\label{tab:overview}
\end{sidewaystable}
